Towards Interactive Intelligence for Digital Humans

We introduce Interactive Intelligence, a novel paradigm of digital human that is capable of personality-aligned expression, adaptive interaction, and self-evolution. To realize this, we present Mio (Multimodal Interactive Omni-Avatar), an end-to-end framework composed of five specialized modules: Thinker, Talker, Face Animator, Body Animator, and Renderer. This unified architecture integrates cognitive reasoning with real-time multimodal embodiment to enable fluid, consistent interaction. Furthermore, we establish a new benchmark to rigorously evaluate the capabilities of interactive intelligence. Extensive experiments demonstrate that our framework achieves superior performance compared to state-of-the-art methods across all evaluated dimensions. Together, these contributions move digital humans beyond superficial imitation toward intelligent interaction.

==> sec/01.intro_old.tex <==
\section{Introduction}

\subsection{Motivation}

Most existing digital humans are still based on imitation rather than genuine understanding of interaction logic. Current workflows typically rely on general-purpose multimodal generative models, such as Veo3, Kling, Wan2.x, or Sora2 which are trained on massive audiovisual corpora. Artists exploit these priors through extensive prompt engineering, large-scale video sampling, and heavy post-production (e.g., lip synchronization and compositing with third-party software).

While such processes significantly reduce the production time compared with traditional CG pipelines, they remain fundamentally limited. What these AI-driven characters produce are not authentic, autonomous behaviors, but rather simplified imitations or rule-based scripted control systems. They lack the ability to capture and reason about the underlying logic of human interaction.

From the perspective of an NPC as an \textbf{individual agent}, situated in a narrative context with a personalized identity, genuine interactive intelligence requires the following capabilities:

\begin{itemize}
    \item \textbf{Personality-aligned expression:} 
    \begin{itemize}
        \item \textit{Lexical choice:} individualized word usage and phrasing
        \item \textit{Voice:} distinctive timbre, pitch, and prosody
        \item \textit{Facial expressions:} personalized affective responses
        \item \textit{Body movements:} coherent, character-specific motion patterns
        \item \textit{Rendering style:} consistent appearance, clothing, and aesthetic identity
    \end{itemize}
    
    \item \textbf{Human--NPC interaction:} The NPC should demonstrate active listening and adaptive feedback based on the interlocutor’s speech style and intent. This process should emerge from understanding rather than pre-scripted rules.
    
    \item \textbf{Environment interaction:} The NPC should perceive its surroundings and plan plausible, context-aware actions.
    
    \item \textbf{Robustness to adversarial prompts:} For example, hallucinations such as ``asking Harry Potter to compose Tang poetry'' should not occur, since they violate narrative and temporal constraints.
    
    \item \textbf{Self-evolution:} The NPC should be able to adapt and improve through interaction feedback, autonomously adjusting behavior and refining task planning---a hallmark of growth and learning.
\end{itemize}

To pursue this vision, our work makes the following contributions:
\begin{enumerate}
    \item We propose a foundational paradigm that cascades \textbf{voice, facial expression, body motion, rendering, and a thinker module}, providing digital humans with fundamental expressive and reasoning abilities.
    \item We introduce \textbf{FLUID}, a purpose-built dataset designed to facilitate the learning of interactive intelligence.
    \item We develop a \textbf{benchmark evaluation framework} that systematically measures progress in interactive AI.
\end{enumerate}

Together, these contributions lay a practical foundation toward building digital humans with genuine \textbf{end-to-end interactive intelligence}.


% \begin{figure}
%   \centering
%   % \fbox{\rule[-.5cm]{4cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
% \includegraphics[height=2cm]{figures/figure1.svg}
%   \caption{Sample figure caption.}
%   \label{fig:fig1}
% \end{figure}

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1\textwidth]{figures/story1.pdf}
%   \caption{
%     \textbf{Context-aware and self-adaptive interaction process between digital human MIO and the Player.}
%     MIO dynamically reacts to the Player’s behavior through a sequence of interactive states 
%     (\textit{Dancing} $\rightarrow$ \textit{Scared} $\rightarrow$ \textit{Sad} $\rightarrow$ \textit{Happy}). 
%     Each response is contextually appropriate — her tone, prosody, facial expressions, body gestures, and rendering style 
%     are all aligned with the conversational and emotional context. 
%     As shown at \textbf{State 2 (Scared)}, the \textit{Thinker} module interprets the Player’s utterance and overall situation, 
%     then decides the multimodal control signals for the \textit{Talker} (speech synthesis), 
%     \textit{Face Animator}, \textit{Body Animator}, and \textit{Renderer} to generate coherent voice, emotion, and motion expressions. 
%     Meanwhile, the \textit{Thinker} continuously learns the Player’s preferences and personality traits, 
%     updating MIO’s internal model to produce more adaptive, personalized, and natural interactions in future dialogues.
%     }
%   \label{fig:story}
% \end{figure}



==> sec/FLUIDdata.tex <==
\section{FLUID Dataset}

The novelty of our \textbf{FLUID dataset} lies in two major aspects:

\begin{enumerate}
    \item \textbf{Closer to realistic interactive scenarios.} 
    Unlike existing datasets (e.g., Meta’s dataset) that mostly simulate two participants engaged in remote, disjoint conversations without physical embodiment, FLUID captures richer and more natural human interactions. In particular, it incorporates \textbf{action-based interactions} and \textbf{action interruptions}, which are critical for modeling dynamic and fluid exchanges in real-world communication.
    
    \item \textbf{Support for multimodal close interaction and 3D reconstruction.}
    Current datasets lack the ability to support 3D reconstruction and do not include physical interactions such as gestures, expressions, or proximity-based behaviors. FLUID is designed as an \textbf{extended version of Harmony4D}, enriched with \textbf{dialogue and close-proximity interactions} between participants. This extension is essential for training AI systems capable of learning \textbf{action- and expression-driven interaction} beyond mere speech exchange.
\end{enumerate}

By introducing these innovations, FLUID provides a unique benchmark for advancing digital humans toward more \textbf{embodied, multimodal, and contextually grounded interaction intelligence}.

